Global Attention for Name Tagging

Many name tagging approaches use local contextual information with much success, but fail when the local context is ambiguous or limited. We present a new framework to improve name tagging by utilizing local, document-level, and corpus-level contextual information. We retrieve document-level context from other sentences within the same document and corpus-level context from sentences in other topically related documents. We propose a model that learns to incorporate document-level and corpus-level contextual information alongside local contextual information via global attentions, which dynamically weight their respective contextual information, and gating mechanisms, which determine the influence of this information. Extensive experiments on benchmark datasets show the effectiveness of our approach, which achieves state-of-the-art results for Dutch, German, and Spanish on the CoNLL-2002 and CoNLL-2003 datasets.

==> 2universal.tex <==
\section{Starting Time: Language Universals}
\label{section_universal}

First we use some language universal rules, gazetteers and patterns to generate a binary feature vector $F=\{f_1,f_2,...\}$ for each token. Table~\ref{tab:universal_tagger} shows these features along with examples. An identification rule is $r_I=\langle T_I,f=\{f_a,f_b,...\}\rangle $ where $T_I$ is a ``B/I/O'' tag to indicate the beginning, inside or outside of a name, and $\{f_a,f_b,...\}$ is a set of selected features. If the features are all matched, the token will be tagged as $T_I$. Similarly, a classification rule is $r_C=\langle T_C,f=\{f_a,f_b,...\}\rangle $, where $T_C$ is ``Person/Organization/Location''.
%We generate a list of identification rules $R_I=\{r_{i1},r_{i2},...\}$ and a list of classification rules $R_C=\{r_{c1},r_{c2},..\}$. Rules in the list 
These rules are triggered in order, and some examples are as follows: $\langle$B, \{AllUppercased\}$\rangle$, $\langle$PER, \{PersonGaz\}$\rangle $, $\langle $ORG, \{Capitalized, LongLength\}$\rangle $, etc.
%For example, if $r_{i1}$ is satisfied, the term is tagged and the identification for this term stops. Else, it checks $r_{i1}$. If all rules fail, term is tagged as ``O'' or ``NoneType''.
%Some examples of tagging rules are: 

% \begin{itemize}
% \setlength\itemsep{-0.3em}
% \item {\footnotesize $<$B, \{AllUppercased\}$>$}
% %\item {\footnotesize $<$B, \{Capitalized, non-TF-IDF\}$>$}
% \item {\footnotesize $<$PER, \{PersonGaz\}$>$}
% \item {\footnotesize $<$ORG, \{Capitalized, LongLength\}$>$}
% %\item {\footnotesize $<$ORG, \{MixedCase\}$>$}
% \end{itemize}
% \vspace{-0.5em}

%\todo{cut the table down to a few bullets}

\begin{table*}[h!t]
\centering
\scriptsize
% \footnotesize
\begin{tabular}{p{1.2cm}p{14.5cm}}
\toprule
Features & Examples (Feature name is underlined) \\ \hline
in English Gazetteer & - \underline{\textbf{PerGaz}}: person ($472,765$); \underline{\textbf{LocGaz}}: location ($211,872$); \underline{\textbf{OrgGaz}}:  organization ($124,403$); \underline{\textbf{Title}} ($889$); \underline{\textbf{NoneName}} ($2,380$). \\
% & - \underline{\textbf{Title}}: in title gazetteer ($889$); \underline{\textbf{NoneName}}: in non-name gazetteer ($2,380$). \\ \\
Case & - \underline{\textbf{Capitalized}}; - \underline{\textbf{AllUppercased}}; - \underline{\textbf{MixedCase}} \\
%\multirow{2}{*}{} & - \underline{\textbf{AllUppercased}}: word is all uppercased \\
% & - \underline{\textbf{MixedCase}}: word is mixed case \\ \\
Punctuation & - \underline{\textbf{IternalPeriod}}: includes an internal period \\
Digit & - \underline{\textbf{Digits}}: consisted of digits \\
Length & - \underline{\textbf{LongLength}}: a name including more than 4 tokens is likely to be an ORG \\
TF-IDF & - \underline{\textbf{TF-IDF}}: if a capitalized word appears at the beginning of a sentence, and has a low TF-IDF, then it's unlikely to be a name \\
Patterns & - \underline{\textbf{Pattern1}}: ``\textit{Title} $\langle$ PER Name $\rangle$'' \\
\multirow{2}{*}{} & - \underline{\textbf{Pattern2}}: ``$\langle PER Name\rangle , 00 *, $'' where $00$ are two digits \\
 & - \underline{\textbf{Pattern3}}: ``$[\langle Name_i\rangle  ...], \langle Name_n-1\rangle \langle single term\rangle \langle Name_n\rangle $'' where all names have the same type. \\
Multi-occurrences & - \underline{\textbf{MultipleOccurrence}}: If a word appears in both uppercased and lowercased forms in a single document, it's unlikely to be a name. \\ \bottomrule
\end{tabular}
\caption{Universal Name Tagger Features}
\label{tab:universal_tagger}
\end{table*}




==> 3.1overview.tex <==
\subsection{Approach Overview}


Figure~\ref{fig:expectation_overview} illustrates our overall approach of acquiring various expectations, by simulating the strategies human players adopted during the Tibetan Room game. Next we will present details about discovering expectations from each source.

\graphicspath { {./fig/} }
\begin{figure}[ht]
 \centering
   \includegraphics[width=0.5\textwidth]{expectation_overview}
   \caption{Expectation Driven Name Tagger Overview}
   \label{fig:expectation_overview}
\end{figure}

==> 3.2survey.tex <==
\subsection{Survey with Native Speaker}

The best way to understand a language is to consult people who speak it. %Our expectation discovery framework includes 
We introduce a human-in-the-loop process to acquire knowledge from native speakers. %However, in the mission of disaster rescue, time is so valuable that it's impossible to spend much time on questioning people in a disaster. Our goal is to gather precise, informative and high quality knowledge in an hour.
To meet the needs in the emergent setting, we design a comprehensive survey that aims to acquire a wide-range of IL-specific knowledge from native speakers in an efficient way. 
%capture language knowledge as broad as possible in an efficient way. 
The survey categorizes questions and organizes them into a tree structure, so that the order of questions is chosen based on the answers of previous questions. The survey answers are then automatically translated into rules, patterns or gazetteers in the tagger. Some example questions are shown in Table~\ref{tab:survey_questions}.
%. Question presented to native speaker are chosen based on answers of previous questions.

%XXX sample questions

\begin{table*}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{p{20cm}}
\toprule
\textbf{True/False Questions} \\
1. The letters of this language have upper and lower cases \\
2. The names of people, organizations and locations start with a capitalized (uppercased) letter \\
3. The first word of a sentence starts with a capitalized (uppercased) letter \\
4. Some periods indicate name abbreviations, e.g., St. = Saint, I.B.M. = International Business Machines. \\
5. Locations usually include designators, e.g., in a format like “country United states”, “city Washington” \\
6. Some prepositions are part of names \\ \hline
\textbf{Text input} \\
1. Morphology: please enter preposition suffixes as many as you can (e.g. ``’da'' in ``Ankara’da yaşıyorum (I live in Ankara)'' is a preposition suffix which means ``in''). \\ \hline
\textbf{Translation}\\
1. Please translate the following English words and phrases: \\
- organization suffix: agency, group, council, party, school, hospital, company, office, ... \\ 
%- time expression: January, February, March, April, May, June, July, August, September, October, November, December, Monday, Tuesday, Wednesday, Thursday, Friday, Saturday, Sunday... \\
- time expression: January, ..., December; Monday, ..., Sunday; ... \\
\bottomrule
\end{tabular}
}
\caption{Survey Question Examples}
\label{tab:survey_questions}
\end{table*}







==> 3.3monolingual.tex <==
\subsection{Mono-lingual Expectation Mining}

%\todo{Add manual filtering step, write the number of patterns before and after filtering}


We use a bootstrapping method to acquire IL patterns from unlabeled mono-lingual IL documents. %Patterns are used for name classification. 
Following the same idea in \cite{agichtein2000snowball,collins1999unsupervised}, we first use names identified by high-confident rules as seeds, and 
%find occurrences of the seeds in mono-lingual text. Then the system generates 
generalize patterns from the contexts of these seeds. Then we evaluate the patterns and apply high-quality ones to find more names as new seeds. This process is repeated iteratively~\footnote{We empirically set the number of iterations as 2 in this paper.}.
% New discovered names are regarded as new seeds. Then the system mines more patterns and names iteratively.

We define a pattern as a triple $\langle left, name, right\rangle$, where $name$ is a name, left and right\footnote{$left$ and $right$ are the context three tokens before and after the name} are context vectors with weighted terms (the weight is computed based on each token's tf-idf score). For example, from a Hausa sentence ``\emph{\textbf{gwamnatin kasar Sin ta} samar wa kasashen yammacin Afirka ... (the Government of China has given ... products to the West African countries)}'', we can discover a pattern:
\vspace{-0.2em}
\begin{itemize}[leftmargin=*]
\small
\setlength\itemsep{-0.5em}
\item $left$: $\langle$\textbf{gwamnatin} (goevernment), 0.5$\rangle$, $\langle$\textbf{kasar} (country), 0.6$\rangle$
\item $name$: $\langle$\textbf{Sin} (China), 0.5$\rangle$
\item $right$: $\langle$\textbf{ta} (by), 0.2$\rangle$
\end{itemize}
This pattern matches strings like ``\emph{gwamnatin kasar Fiji ta (by the government of Fiji)}''. 

%In the example above, the number associated with each term is a function of the frequency of the term in the corresponding context. 
%The vectors $l_P$ and $r_P$ are composed of terms with weights representing the $left$ and $right$ contexts. 
For any two triples $t_i=\langle l_i, name_i, r_i \rangle$ and $t_j=\langle l_j, name_j, r_j \rangle$, we comput e their similarity by:
\vspace{-0.3em}
\begingroup\makeatletter\def\f@size{10}\check@mathfonts
\small
\[
Sim(t_i, t_j)=l_i\cdot l_j+r_i\cdot r_j
\]
\endgroup
% \vspace{-0.5em}
%Triples are considered as similar if their similarity is over a threshold $\tau_{sim}$.
We use this similarity measurement to cluster all triples and select the centroid triples in each cluster as candidate patterns.

%Generating good patterns are challenging. For example, pattern $<\{\}, \{<PERSON>\}, \{<ya(said), 0.7>, <ce(said)>, 0.7\}>$ generated from text occurrence ``shugaban Obama ya ce (President Obama said)'' may lead to name classification error in ``Har yanzu ana tantance yawan waɗanda su ka mutu da waɗanda su ka sami rauni, \textbf{YouAn} \underline{ya ce}. (The number of dead and injured were still being tallied, hospital YouAn said.)'' where ``YouAn'' is incorrectly tagged as PERSON. ``Bad'' discovered by ``Bad'' patterns will introduce more ``Bad'' patterns in next iteration. 

Similar to~\cite{agichtein2000snowball}, we evaluate the quality of a candidate pattern P by:
\vspace{-0.5em}
\begingroup\makeatletter\def\f@size{10}\check@mathfonts
% * <boliangzhang85@gmail.com> 2016-05-28T15:42:01.079Z:
%
% > begingroup
%
% ^.
\small
\[
Conf(P)=\frac{P_{positive}}{(P_{positive}+P_{negative})}
\]
\endgroup
% \vspace{-0.5em}
,where $P_{positive}$ is the number of positive matches for $P$ and $P_{negative}$ is the number of negative matches. Due to the lack of syntactic and semantic resources to refine these lexical patterns, we set a conservative confidence threshold 0.9.



==> 3.4crosslingual.tex <==
\subsection{Cross-lingual Expectation Projection}
\label{section_projection}

Name tagging research has been done for high-resource languages such as English for over twenty years, so we have learned a lot about them. We collected 1,362 %\todo{and the number of English patterns} 
patterns from English name tagging literature. Some examples are listed below: % (morphology is removed): \todo{list sample English patterns in a table}

\begin{itemize}
\setlength\itemsep{-0.5em}
\item {\scriptsize $\langle\{\}, \{PER\}, \{<say>, <.>\}\rangle$}
%\item {\scriptsize $\langle\{\}, \{PER\}, \{<send>, <to>\}\rangle$}
\item {\scriptsize $\langle\{<headquarter>, <in>\}, \{LOC\}, \{\}\rangle$}
\item {\scriptsize $\langle\{<secretary>, <of>\}, \{ORG\}, \{\}\rangle$}
\item {\scriptsize $\langle\{<in>, <the>\}, \{LOC\}, \{<area>\}\rangle$}
\end{itemize}

Besides the static knowledge like patterns, we can also dynamically acquire expected names from topically-related English documents for a given IL document. We apply the Stanford name tagger~\cite{finkel2005incorporating} to the English documents to obtain a list of expected names. Then we translate the English patterns and expected names to IL. When there is no human constructed English-to-IL lexicon available, we derive a word-for-word translation table from a small parallel data set using the GIZA++ word alignment tool~\cite{och2003systematic}. 
%For example, the pattern ``\emph{Prime Minister <PERSON>}'' is translated to Bengali ``\emph{{\bengalifont প্রধানমন্ত্রী} <PERSON>}''. 
We also convert IL text to Latin characters based on Unicode mapping\footnote{http://www.ssec.wisc.edu/~tomw/java/unicode.html}, and then apply Soundex code~\cite{mortimer1995soundex,raghavan2004using} to find the IL name equivalent that shares the most similar pronunciation as each English name. For example, the Bengali name ``\emph{\begin{bengali}টনি ব্লেয়ার\end{bengali}}" and ``\emph{Tony Blair}'' have the same Soundex code ``\emph{T500 B460}''.



==> 3.5KB.tex <==
\subsection{Mining Expectations from KB}

In addition to unstructured documents, we also try to leverage structured English knowledge bases (KBs) such as DBpedia\footnote{http://dbpedia.org}. 
%Table~\ref{table:kb_entry} presents the number of entries in DBpedia for some low-resource languages. 
Each entry is associated with a set of types such as \texttt{Company}, \texttt{Actor} and \texttt{Agent}. We utilize the Abstract Meaning Representation corpus~\cite{Banarescu2013} which contains both entity type and linked KB title annotations, to automatically map $9,514$ entity types in DBPedia to three main entity types of interest: Person (PER), Location (LOC) and Organization (ORG). 

Then we adopt a language-independent cross-lingual entity linking system~\cite{Wang2015} to link each IL name mention to English DBPedia. This linker is based on an unsupervised quantified collective inference approach. It constructs knowledge networks from the IL source documents based on entity mention co-occurrence, and knowledge networks from KB. Each IL name is matched with candidate entities in English KB using name translation pairs derived from inter-lingual KB links in Wikipedia and DBPedia. We also apply the word-for-word translation tables constructed from parallel data as described in Section~\ref{section_projection} to translate some uncommon names. Then it performs semantic comparison between two knowledge networks based on three criteria: salience, similarity and coherence. Finally we map the DBPedia types associated with the linked entity candidates to obtain the entity type for each IL name.


% \begin{table}[hbtp]
% %\footnotesize
% \scriptsize
% \centering
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{ccccccccc}
% \toprule
% Bengali & Hausa & Tamil & Tagalog \\
% 40.0K & 1.4K & 82.8K & 64.2K \\ \hline
% Thai & Turkish & Yoruba & English \\
% 99.3K & 258.8K & 31.1K & 5,047.9K \\
% %Bengali & Hausa & Tamil & Tagalog & Thai & Turkish & Yoruba & English\\
% %40.0K & 1.4K & 82.8K & 64.2K & 99.3K & 258.8K & 31.1K & 5,047.9K \\
% \bottomrule
% \end{tabular}
% % }
% \caption{\# of Entries in KB} 
% \label{table:kb_entry}
% \vspace{-0.8em}
% \end{table}




==> 3expectation.tex <==


\input{3.1overview}
\input{3.2survey}
\input{3.3monolingual}
\input{3.4crosslingual}
\input{3.5KB}




==> 4active.tex <==
\section{Supervised Active Learning}

We anticipated that not all expectations can be encoded as explicit rules and patterns, or covered by projected names, therefore for comparison we introduce a supervised method with pool-based active learning to learn implicit expectations (features, new names, etc.) directly from human data annotation. %preprocessing. 
We exploited basic lexical features including ngrams, adjacent tokens, casing information, punctuations and frequency to train a Conditional Random Fields (CRFs)~\cite{Lafferty2001} based model through active learning~\cite{settles2010active}.
%Features are listed in table~\ref{tab:active_feature}
%\begin{table}
%\resizebox{\columnwidth}{!}{
%\begin{tabular}{lp{6cm}}
%\toprule
%\textbf{Features} & \textbf{Descriptions} \\
%\hline
%n-gram & unigram, bigram and trigram \\ \hline
%adjacent tokens & tokens before and after \\ \hline
%case & capitalized, all capitalized and mixed case \\ \hline
%special character & contains hyphen, apostrophe, digit and period \\ \hline
%frequency & frequency in training corpus \\
%\bottomrule
%\end{tabular}
%}
%\caption{Active Learning Tagger Features}
%\label{tab:active_feature}
%\end{table}

%\todo{List features}

We segment documents into sentences and use each sentence as a training unit. Let $\boldsymbol{\mathrm{x}}_b^*$ be the most informative instance according to a query strategy $\phi(\boldsymbol{\mathrm{x}})$, which is a function used to evaluate each instance $\boldsymbol{\mathrm{x}}$ in the unlabeled pool $U$. Algorithm~\ref{alg:active_learning} illustrates the procedure.
%provides a sketch of the scenario.

\begin{algorithm}
\footnotesize
\caption{Pool-based Active Learning}\label{alg:active_learning}
\begin{algorithmic}[1]
\State $L\gets$ labeled set, $U\gets$ unlabeled pool
\State $\phi(\cdot)\gets$ query strategy, $B\gets$ query batch size
\State $M\gets$ maximum number of tokens
\While{Length($L$)$<M$}
\State $\theta=\mathrm{train}(L)$;
\For{$b \in \{1,2,...,B\}$}
\State $\boldsymbol{\mathrm{x}}_b^*=\arg\max_{x\in U}\phi(\boldsymbol{\mathrm{x}})$
\State $L=L\cup\{\boldsymbol{\mathrm{x}}_b^*, \mathrm{label}(\boldsymbol{\mathrm{x}}_b^*)\}$
\State $U=U-\boldsymbol{\mathrm{x}}_b^*$
\EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}


\newcite{Jing2004} proposed an entropy measure for active learning for image retrieval task. We compared it with other measures proposed by~\cite{settles2008analysis} and found that \textbf{sequence entropy (SE)} is most effective for our name tagging task. We use $\phi^{SE}$ to represent how informative a sentence is:\\
%,  %$\phi^{SE}$ is 
%and it's defined as:\\
{\footnotesize{$$\phi^{SE}(\boldsymbol{\mathrm{x}})=-\sum_{t=1}^{T}\sum_{m=1}^{M}P_\theta(y_t=m)logP_\theta(y_t=m)$$}}, where T is the length of $\boldsymbol{\mathrm{x}}$, $m$ ranges over all possible token labels and $P_\theta(y_t=m)$ is the probability when $y_t$ is tagged as $m$.





==> 5prioritize.tex <==
%\section{Prioritize and Compose Expectations}
\section{Cost-aware Combination}
\label{section_combination}

%\todo{Add in details about confidence estimation, combination method, etc.}

A new requirement for IL name tagging is a \textbf{Linguistic Workflow Generator}, which can generate an activity schedule to organize and maximize the use of acquired expectations to yield optimal F-scores within given time bounds. Therefore, the input to the IL name tagger is not only the test data, but also a time bound for development (1 hour, 2 hours, 24 hours, 1 week, 1 month, etc.).

Figure~\ref{fig:overview} illustrates our cost-aware expectation composition approach. Given some IL documents as input, as the clock ticks, the system delivers name tagging results at time 0 (immediately), time 1 (e.g., in one hour) and time 2 (e.g., in two hours). At time 0, name tagging results are provided by the  universal tagger described in Section~\ref{section_universal}. 
%Since both expectation learning and supervised active learning require the contributions from native speakers, we need to compose them carefully. For example, 
During the first hour, we can either ask the native speaker to annotate a small amount of data for supervised active learning of a CRFs model, or fill in the survey to build a rule-based tagger. 
%To investigate which one is more promising, we conducted experiments for comparison (Section~\ref{section_overallexpt}). 
We estimate the confidence value of each expectation-driven rule based on its precision score on a small development set of ten documents. Then we apply these rules in the priority order of their confidence values. When the results of two taggers are conflicting on either mention boundary or type, if the applied rule has high confidence we will trust its output, otherwise adopt the CRFs model's output.

\graphicspath { {./fig/} }
\begin{figure*}[ht]
 \centering
   \includegraphics[width=0.99\textwidth]{composition_overview}
   \caption{Cost-aware Expectation Composition}
   \label{fig:overview}
\end{figure*}





==> 6.1data.tex <==
\subsection{Data}
% list the data sets from all kinds of languages
%In this paper, 
We evaluate our framework on seven low-resource incident languages: Bengali, Hausa, Tagalog, Tamil, Thai, Turkish and Yoruba, using the ground-truth name tagging annotations from the DARPA LORELEI program~\footnote{http://www.darpa.mil/program/low-resource-languages-for-emergent-incidents}. Table~\ref{TableStats} shows data statistics.

\begin{table}
\centering
\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{p{1cm}p{1cm}p{1cm}p{1cm}p{1.2cm}p{1.5cm}}
\toprule
\textbf{Language} & \textbf{IL Test Docs} & \textbf{Name} & \textbf{Unique Name} & \textbf{IL Dev. Docs} & \textbf{IL-English Docs} \\ \hline
Bengali	& 100 & 4,713 & 2,820 & 12,495 & 169 \\ 
Hausa	& 100 & 1,619 & 950 & 13,652 & 645 \\ 
Tagalog	& 100 & 6,119 & 3,375 & 1,616 & 145 \\ 
Tamil	& 100 & 4120 & 2,871 & 4,597 & 166 \\ 
Thai	& 100 & 4,954 & 3,314 & 10,000 & 191 \\ 
Turkish	& 100 & 2,694 & 1,323 & 10,000 & 484 \\ 
Yoruba	& 100 & 3,745 & 2,337 & 427 & 252 \\
\bottomrule
\end{tabular}
}
\caption{Data Statistics} \label{TableStats}
\end{table}



==> 6.2overall.tex <==
\subsection{Cost-aware Overall Performance}
\label{section_overallexpt}

We test with three checking points: starting time, within one hour, and within two hours. Based on the combination approach described in Section~\ref{section_combination}, we can have three possible combinations of the expectation-driven learning and supervised active learning methods during two hours: (1) expectation-driven learning + supervised active learning; (2) supervised active learning + expectation-driven learning; and (3) supervised active learning for two hours. Figure~\ref{fig:combination_fig} compares the overall performance of these combinations for each language.

We can see that our approach is able to rapidly set up a name tagger for an IL and achieves promising performance. During the first hour, there is no clear winner between expectation-driven learning or supervised active learning. But it's clear that supervised active learning for two hours is generally not the optimal solution. Using Hausa as a case study, we take a closer look at the supervised active learning curve as shown in Figure~\ref{fig:learning_curve}. We can see that supervised active learning based on simple lexical features tends to converge quickly. 
%In other words, a supervised active learner based on simple lexical features has its own limitations. 
As time goes by it will reach its own upper-bound of learning and generalizing linguistic features. In these cases our proposed expectation-driven learning method can compensate by providing more explicit and deeper IL-specific linguistic knowledge.



%\todo{add a specific point, it starts to converge at 2 hours....} 
% \todo{Add new figure, add discussion, example, analysis; give examples to show some time explicit expectations work, sometimes we need to rely on active learning}
%%XXX and how to prioritize different resources; show the priority is convincing, and it works for all languages


\graphicspath { {./fig/} }
\begin{figure*}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{ben}
  \caption{Bengali}
  \label{fig:combination_ben}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{hau}
  \caption{Hausa}
  \label{fig:combination_hau}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{tam}
  \caption{Tamil}
  \label{fig:combination_tam}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{tgl}
  \caption{Tagalog}
  \label{fig:combination_tgl}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{tha}
  \caption{Thai}
  \label{fig:combination_tha}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{tur}
  \caption{Turkish}
  \label{fig:combination_tur}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=.5\linewidth]{yor}
  \caption{Yoruba}
  \label{fig:combination_yor}
\end{subfigure}
\caption{Comparison of methods combining expectation-driven learning and supervised active learning given various time bounds}
\label{fig:combination_fig}
\end{figure*}


%\todo{add Hausa active learning curve here}
\graphicspath { {./fig/} }
\begin{figure}
 \centering
   \includegraphics[width=1.0\linewidth]{learning_curve}
   \caption{Hausa Supervised Active Learning Curve}
   \label{fig:learning_curve}
\end{figure}

% \begin{figure}[!htb]
% \ContinuedFloat
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{yor}
%   \caption{Yoruba}
%   \label{fig:combination_yor}
% \end{subfigure}
% \caption{Cost-aware Overall Performance (continued)}
% \label{fig:fig}
% \vspace{-0.6em}
% \end{figure}




==> 6.3expectationdriven.tex <==
\subsection{Comparison of Expectation Discovery Methods}
%\todo{Add break down results for different types of expectations; add analysis and examples}
Table~\ref{tab:expectation_breakdown} shows the performance gain of each type of expectation acquisition method. IL gazetteers covered some common names, especially when the universal case-based rules failed at identifying names from non-Latin languages. IL name patterns were mainly effective for classification. For example, the Tamil name ``{\deffont கத்தோலிக்கன் சிரியன் வங்கியில} (Catholic Syrian Bank)'' was classified as an organization because it ends with an organization suffix word ``{\deffont வங்கியில}(bank)''. The patterns projected from English were proven very effective at identifying name boundaries. For example, some non-names such as titles are also capitalized in Turkish, so simple case-based patterns produced  many spurious names. But projected patterns can fix many of them. In the following Turkish sentence, ``\emph{Ancak Avrupa Birliği Dış İlişkiler Sorumlusu Catherine Ashton,...(But European Union foreign policy chief Catherine Ashton,...)}", among all these capitalized tokens, after we confirmed ``\emph{Avrupa Birliği (European Union)}" as an organization and ``\emph{Dış İlişkiler Sorumlusu (foreign policy chief)}" as a title, we applied a pattern projected from English ``\emph{[Organization] [Title] [Person]}" and successfully identified ``\emph{Catherine Ashton}" as a person. Cross-lingual entity linking based typing successfully enhanced classification accuracy, especially for languages where names often appear the same as their English forms and so entity linking achieved high accuracy. For example, ``\emph{George Bush}" keeps the same in Hausa, Tagalog and Yoruba as English. 


\begin{table*}
\centering
\small
\begin{tabular}{lccccccc}
\toprule
\textbf{Methods} & \textbf{Bengali} & \textbf{Hausa} & \textbf{Tamil} & \textbf{Tagalog} & \textbf{Thai} & \textbf{Turkish} & \textbf{Yoruba} \\ \hline
Universal Rules & 4.1 & 26.5 & 0.0 & 30.2 & 2.2 & 12.4 & 17.1 \\
+IL Gazetteers & 29.7 & 32.1 & 21.8 & 34.3 & 18.9 & 17.3 & 26.9 \\
+IL Name Patterns & 31.2 & 33.8 & 22.9 & 35.1 & 18.9 & 19.1 & 28.0 \\
+IL to English Lexicons & 31.3 & 35.2 & 24.0 & 38.0 & 20.5 & 19.6 & 29.4 \\
+IL Survey with Native Speaker & 34.1 & 40.6 & 25.6 & 45.9 & 21.6 & 39.3 & 30.2 \\
+KB Linking based Typing & 34.8 & 48.3 & 26.0 & 51.3 & 21.7 & 43.6 & 36.0 \\ \bottomrule
\end{tabular}
\caption{Contributions of Various Expectation Discovery Methods (F-score \%) } 
\label{tab:expectation_breakdown}
\end{table*}




==> 6.4activelearning.tex <==
\subsection{Impact of Supervised Active Learning}

Figure~\ref{fig:active_vs_passive} shows the comparison of supervised active learning and passive learning (random sampling in training data selection). We asked a native speaker to annotate Chinese news documents in one hour, and estimated the human annotation speed approximately as 7,000 tokens per hour. Therefore we set the number of tokens as 7,000 for one hour, and 14,000 for two hours. We can clearly see that supervised active learning significantly outperforms passive learning for all languages, especially for Tamil, Tagalog and Yoruba. Because of the rich morphology in Turkish, the gain of supervised active learning is relatively small because simple lexical features cannot capture name-specific characteristics regardless of the size of labeled data. For example, some prepositions (e.g., ``\emph{nin (in)}'') can be part of the names, so it's difficult to determine name boundaries, such as ``\emph{<ORG Ludian bölgesi \textbf{hastanesi}>\textbf{nin} (in <ORG Ludian Hospital>)}''

%, times partial token is identified as a name during annotation process, e.g. ``Ludian bölgesi hastanesinin (in Ludian Hospital)'' has annotation ``<ORG Ludian bölgesi hastanesi>nin (in Ludian Hospital)'' where ``nin'' is left out. General features in the name tagger are ineffective in this case. Therefore, performance gain of active learning for Turkish is trivial.

\graphicspath { {./fig/} }
\begin{figure}
 \centering
   \includegraphics[width=.48\textwidth]{active_vs_passive_fig}
   \caption{Active Learning vs. Passive Learning (\%)}
   \label{fig:active_vs_passive}
\end{figure}




==> 6.5discussion.tex <==
\subsection{Remaining Error Analysis}

\begin{table}[hbtp]
\centering
\resizebox{\columnwidth}{!}{
	\begin{tabular}{ccccccc}
	    \toprule
		\multirow{2}{*}{\textbf{Language}} & \multicolumn{4}{c}{\textbf{Identification F-score}} & \multirow{2}{2.1cm}{\centering \textbf{Typing Accuracy*}} & \multirow{2}{1.5cm}{\centering \textbf{Overall F-score}} \\
		\cmidrule(l){2-5}
		& \textbf{PER} & \textbf{ORG} & \textbf{LOC} & \textbf{All} & & \\ \hline
		Bengali & 51.0 & 32.7 & 54.3 & 48.5 & 84.1 & 40.7 \\
		Hausa & 51.8 & 36.6 & 63.3 & 55.1 & 93.6 & 51.6 \\
		Tamil & 40.4 & 16.4 & 46.8 & 39.2 & 86.2 & 33.8 \\
		Tagalog & 71.6 & 65.2 & 73.9 & 70.1 & 92.8 & 65.1 \\
		Thai & 48.5 & 21.8 & 72.8 & 48.6 & 72.0 & 35.0 \\
		Turkish & 64.3 & 41.3 & 73.0 & 63.1 & 69.1 & 43.6 \\
		Yoruba & 69.3 & 38.3 & 60.0 & 57.2 & 82.3 & 47.1 \\
		\bottomrule
	\end{tabular}
}
\footnotesize{* typing accuracy is computed on correctly identified names}
\caption{Breakdown Scores}
\label{table:overall_score_breakdown}
\end{table}

Table~\ref{table:overall_score_breakdown} presents the detailed break-down scores for all languages. We can see that name identification, especially organization identification is the main bottleneck for all languages. For example, many organization names in Hausa are often very long, nested or all low-cased, such as ``\emph{makarantar horas da Malaman makaranta ta Bawa Jan Gwarzo (Bawa Jan Gwarzo Memorial Teachers College)}"
%``\emph{cibiyar nazarin aikin magani da horaswa (Institute of Medicine and Training)}" 
 and ``\emph{kungiyar masana'antu da tattalin arziki ta kasar Sin (China's Association of Business and Industry)}". Our name tagger will further benefit from more robust universal word segmentation, rich morphology analysis and IL-specific knowledge. For example, in Tamil ``{\deffont ஃ}" is a visarga used as a diacritic to write foreign sounds, so we can infer a phrase including it  (e.g., ``{\deffont ஹெய்ஃபாவின்} (Haifa)") is likely to be a foreign name. Therefore our survey should be enriched by exercising with many languages to capture more categories of linguistic phenomena.
 


%In Tamil, the visarga is called āytam, written ஃ. Apart from a modern use as a diacritic to write foreign sounds, it is archaic and employed only in idiomatic and fossilized words such as அஃது(adhu - "there"), இஃது (idhu - "here") etc. It is mentioned in the earliest available Tamil grammatical treatise, Tolkāppiyam (1:1:2), where it is categorized as an allophone (cārpezuttu "dependent sound"). As stated by Krishnamurti (Krishnamurti:2003 p154 [1] ) "The properties of āytam, as described by Tolkāppiyam, were: (1) it occurred after a short vowel and before a stop (voiceless), and its place of articulation is like that of the stop. In other words, ஃ assimilates to the following voiceless stop".
 
%  Incorrect tokenization results in boundary errors in identification. For example, 
%  \begin{thai}
% \XeTeXlinebreaklocale "th"
% \raggedright
% ชาวปาเลสไตน์กล่าวว่า นี่คือสงคราม และนาย\underline{อาราฟัต(Arafat)}ไม่จำเป็นต้องเจรจาเรื่องสันติภาพอีกต่อไป (Palestinians say this is a war , and Mr. Arafat is no need to negotiate a peace anymore.)
% \end{thai}
% " where ``\underline{\begin{thai}อาราฟัต\end{thai}}(Arafat)" is not identified even though we have ``\underline{\begin{thai}อาราฟัต\end{thai}}(Arafat)" in a Thai person name list. A universal word segmenter is helpful in this case. In morphology rich languages, morphological suffixes may lead to identification error, e.g., "Karadeniz kıyısındaki" should be identified "[LOC Karadeniz kıyısı]ndaki " where "ndaki" is a morphological suffix.
 
% Remaining error analysis:
% 1. If sentences are incorrectly segmented, context based features and patterns would fail. A universal sentence segmenter will help in this case.

% 2. Incorrect tokenization results in errors like ``
% \begin{thai}
% \XeTeXlinebreaklocale "th"
% \raggedright
% ชาวปาเลสไตน์กล่าวว่า นี่คือสงคราม และนาย\underline{อาราฟัต(Arafat)}ไม่จำเป็นต้องเจรจาเรื่องสันติภาพอีกต่อไป
% \end{thai}
% " where ``\underline{\begin{thai}อาราฟัต\end{thai}}(Arafat)" is not tagged even though we have ``\underline{\begin{thai}อาราฟัต\end{thai}}(Arafat)" in dictionary. A universal word segmenter is helpful in this case.

% 3. In morphology rich languages, e.g. Turkish, morphology analyzer is important to name tagger. For example, "Karadeniz kıyısındaki" should be tagged "[LOC Karadeniz kıyısı]ndaki " where "ndaki" is a morphological suffix.

% 4. Universal POS tagger and semantic calss tagger are helpful when generating patterns.




==> 6experiment.tex <==
\section{Experiments}

%We evaluated our framework on seven low-resource languages. 
In this section we will present our experimental details, results and observations.

\input{6.1data}
\input{6.2overall}
\input{6.3expectationdriven}
\input{6.4activelearning}
\input{6.5discussion}

==> 7related.tex <==
\section{Related Work}
%\todo{finish a draft for the related work section asap, I need it to finalize the tone for intro}
%\todo{revise, make it sharper}

Name Tagging is a well-studied problem. Many types of frameworks have been used, including rules~\cite{farmakiotou2000rule,nadeau2007survey}, supervised models using monolingual labeled data~\cite{zhou2002named,chieu2002named,rizzo2012nerd,mccallum2003early,LiMcCallum2003}, bilingual labeled data~\cite{li2012joint,kim2012multilingual,che2013named,wang2013joint} or naturally partially annotated data such as Wikipedia~\cite{nothman2013learning}, bootstrapping~\cite{agichtein2000snowball,niu2003bootstrapping,becker2005optimising,wu2009domain,chiticariu2010domain}, and unsupervised learning~\cite{mikheev1999named,mccallum2003early,etzioni2005unsupervised,nadeau2006unsupervised,nadeau2007survey,Ji2009}. 

Name tagging has been explored for many  non-English languages such as in Chinese~\cite{Ji2005,Li2014}, Japanese~\cite{asahara2003japanese,Li2014}, Arabic~\cite{maloney1998tagarab}, Catalan~\cite{carreras2003named}, Bulgarian~\cite{osenova2002combining}, Dutch~\cite{de2002named}, French~\cite{bechet2000tagging}, German~\cite{thielen1995approach}, Italian~\cite{cucchiarelli1998automatic}, Greek~\cite{karkaletsis1999named}, Spanish~\cite{arevalo2002proposal}, Portuguese~\cite{hana2006tagging}, Serbo-croatian~\cite{nenadic2000recognition}, Swedish~\cite{dalianis2001swenam} and Turkish~\cite{tur2003statistical}. However, most of previous work relied on substantial amount of resources such as language-specific rules, basic tools such as part-of-speech taggers, a large amount of labeled data, or a huge amount of Web ngram data, which are usually unavailable for low-resource ILs. In contrast, in this paper we put the name tagging task in a new emergent setting where we need to process a surprise IL within very short time using very few resources. 

The TIDES 2003 Surprise Language Hindi Named Entity Recognition task~\cite{LiMcCallum2003} had a similar setting. A name tagger was required to be finished within a time bound (five days). However, 628 labeled documents were provided in the TIDES task, while in our setting no labeled documents are available at the starting point. Therefore we applied active learning to efficiently annotate about 40 documents for each language and proposed new methods to learn expectations. 
%We explored many different ways of acquiring and encoding expectations from multiple sources. 
The results of the tested ILs are still far from perfect, but we hope our detailed comparison and result analysis can introduce new ideas to balance the quality and cost of name tagging.




==> 8conclusion.tex <==
\section{Conclusions and Future Work}
%\todo{draft punchy take-home messages and interesting future work for me to revise asap}

Name tagging for a new IL is a very important but also challenging task. We conducted a thorough study on various ways of acquiring, encoding and composing expectations from multiple non-traditional sources. 
%such as linguistic knowledge survey with native speakers. %We also proposed a cost-aware combination approach to compose expectations. 
Experiments demonstrate that this framework can be used to build a promising name tagger for a new IL within a few hours. In the future we will exploit broader and deeper entity prior knowledge to improve name identification. We will aim to make the framework more transparent for native speakers so the survey can be done in an automatic interactive question-answering fashion. We will also develop methods to make the tagger capable of active self-assessment to produce the best workflow within time bounds.


